A Verified Architecture for Proofs of Execution on Remote Devices under Full Software Compromise

Modern society is increasingly surrounded by, and accustomed to, a wide range of Cyber-Physical Systems (CPS), Internet-of-Things (IoT), and smart devices. They often perform safety-critical functions, e.g., personal medical devices, automotive CPS and industrial automation (smart factories). Some devices are small, cheap and specialized sensors and/or actuators. They tend to run simple software and operate under control of a more sophisticated central control unit. The latter is responsible for the decision-making and orchestrating the entire system. If devices are left unprotected, consequences of forged sensor readings or ignored actuation commands can be catastrophic, particularly, in safety-critical settings. This prompts the following three questions: (1) How to trust data produced by a simple remote embedded device? and (2) How to ascertain that this data was produced via execution of expected software? Furthermore, (3) Is it possible to attain (1) and (2) under the assumption that all software on the remote device could be modified or compromised? In this paper we answer these questions by designing, proving security of, and formally verifying, VAPE: Verified Architecture for Proofs of Execution. To the best of our knowledge, this is the first of its kind result for low-end embedded systems. Our work has a range of applications, especially, to authenticated sensing and trustworthy actuation, which are increasingly relevant in the context of safety-critical systems. VAPE architecture is publicly available and our evaluation demonstrates that it incurs low overhead, affordable even for lowest-end embedded devices, e.g., those based on MSP430 or ARV ATMega processors.

==> sys-arch.tex <==
\begin{tikzpicture}[node distance=1.5cm, >=stealth]
\tikzset{
  msp430/.style={
    draw,
    rectangle,
    minimum height=5cm,
    minimum width=3cm,
    align=center
  },
  membb/.style={
    draw,
    rectangle,
    minimum height=9cm,
    minimum width=1.5cm,
    align=center
  },
  mem/.style={
    draw,
    rectangle,
    minimum height=.5cm,
    minimum width=1.5cm,
    align=center
  },
  fermat/.style={
    draw,
    rectangle,
    minimum height=3cm,
    minimum width=1.5cm,
    align=center
  },
  arr/.style={->,>=latex'},
  three sided/.style={
        draw=none,
        append after command={
            [shorten <= -0.5\pgflinewidth]
            ([shift={( 0.5\pgflinewidth,-0.5\pgflinewidth)}]\tikzlastnode.north west)
        edge([shift={( 0.5\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south west)            
            ([shift={( 0.5\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south west)
        edge([shift={(-1.0\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south east)       
            ([shift={( 0.5\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south east)
        edge([shift={(-1.0\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.north east)
        }
    }
}
	\node[msp430] (msp) at (0,0) {\large MCU CORE};
        \node[membb] (bb) at (3.5,-2) {\shortstack{MEM.\\\ \\\ \\\ BACK-\\BONE}}; %{\shortstack{M\\E\\M\\O\\R\\Y\\\ \\B\\A\\C\\K\\B\\O\\N\\E}};
        \node[fermat, below = .2cm of bb.south] (fermat) {\hw};
        \node[mem, minimum height=2cm] (srom) at (6, 1.5) {\sw};
        \node[mem, below = .2cm of srom] (krom) {\attkey};
        %\node[mem, below = .2cm of krom, minimum height=1cm] (sstack) {\shortstack{\sw \\ STACK}};
        \node[mem, below = .2cm of krom, minimum height=1cm] (sstack) {\shortstack{\sw \\ STACK \\ (XS)}};
        \node[mem, three sided, below = 0cm of sstack.south, minimum height=3.8cm] (ram) {\shortstack{App. \\ Avail. \\ RAM}};
        \node[mem, below = .2cm of ram, minimum height=4.05cm] (flash) {App. \\ Code};
        
        
        
        \path (msp.east) +(0,.3) coordinate (msp_2);
        \path (msp.east) +(0,-.3) coordinate (msp_3);
        \draw[thick, <-] (msp_2) -- (msp_2 -| bb.west);
        \draw[thick, ->] (msp_3) -- (msp_3 -| bb.west);
        
        \path (msp.south) +(.5,0) coordinate (msp_0);
        \path (msp.south) +(-.5,0) coordinate (msp_1);
        \path (fermat.west) +(0,.5) coordinate (fermat_0);
        \path (fermat.west) +(0,-.5) coordinate (fermat_1);
        \draw[thick, ->] (msp_0) |- (fermat_0); 
        \node[inner sep=5pt,right, fill=white,draw] at ($(msp_0) + (-.75,-2)$) {\small\shortstack{$PC$,\\$irq$,\\$R_{en}$,\\$W_{en}$,\\$D_{addr}$,\\$\dmaen$,\\$\dmaaddr$}};
        %\node[inner sep=6pt,right, fill=yellow,draw,line width=1pt] 
        \draw[thick, <-] (msp_1) |- (fermat_1) ; 
        \node[inner sep=6pt,right, fill=white, draw] at ($(fermat_1) + (-2,0)$) {$reset$};
        
        \path (krom.west) +(0,.1) coordinate (krom_0);
        \path (krom.west) +(0,-.1) coordinate (krom_1);
        \draw[thick, ->] (krom_0) -- (krom_0 -| bb.east);
        \draw[thick, <-] (krom_1) -- (krom_1 -| bb.east);
        
        \path (srom.west) +(0,.1) coordinate (srom_0);
        \path (srom.west) +(0,-.1) coordinate (srom_1);
        \draw[thick, ->] (srom_0) -- (srom_0 -| bb.east); 
        \draw[thick, <-] (srom_1) -- (srom_1 -| bb.east); 
        
        \path (sstack.west) +(0,.1) coordinate (sstack_0);
        \path (sstack.west) +(0,-.1) coordinate (sstack_1);
        \draw[thick, ->] (sstack_0) -- (sstack_0 -| bb.east); 
        \draw[thick, <-] (sstack_1) -- (sstack_1 -| bb.east); 
        
        \path (ram.west) +(0,.1) coordinate (ram_0);
        \path (ram.west) +(0,-.1) coordinate (ram_1);
        \draw[thick, ->] (ram_0) -- (ram_0 -| bb.east); 
        \draw[thick, <-] (ram_1) -- (ram_1 -| bb.east); 
        
        \path (flash.north west) +(0,-.2) coordinate (flash_0);
        \path (flash.north west) +(0,-.4) coordinate (flash_1);
        \draw[thick, ->] (flash_0) -- (flash_0 -| bb.east); 
        \draw[thick, <-] (flash_1) -- (flash_1-| bb.east); 
        
        \draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt] 
        (krom.south east) -- (srom.north east) node [black,midway,xshift=.9cm] {\footnotesize ROM};
        
        \draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt] 
        (ram.south east) -- (sstack.north east) node [black,midway,xshift=.9cm] {\footnotesize RAM};
        
        \draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt] 
        (flash.south east) -- (flash.north east) node [black,midway,xshift=1cm] {\footnotesize FLASH};
\end{tikzpicture}


==> timeline-1col.tex <==
\begin{tikzpicture}[node distance=1.5cm, >=stealth]
	\coordinate (BL)	at (0, 3);		\coordinate[left =4cm  of BL]	 (TL);
	\coordinate (Btcs)	at (0, 2.2);		\coordinate[left =4cm  of Btcs] (Ttcs);
	\coordinate (Btce)	at (0, .8);		\coordinate[left =4cm  of Btce] (Ttce);
	\coordinate (BR)	at (0, 0);		\coordinate[left =4cm  of BR]	 (TR);

	\node[above] at (BL) {\large Prover (\dev)};
	\node[above] at (TL) {\large Verifier (\vrf)};
	\coordinate (Chksum) at ($(Btcs)!0.5!(Btce)$);
	\node [right = .1cm, align=center] at (Chksum) {\small (2) Authenticated \\ \small Integrity Check};
	\coordinate (Verify)	at ($(Ttce)!0.5!(TR)$);
	\node [left =.5cm, align=center] at (Verify) {\small (4) Verify \\ \small Report};

	\draw[line width = .3cm, color=red!50]	(BL) -- (BR);
	\draw[line width = .3cm, color=blue!50] (TL) -- (TR);
	\coordinate (ReqStart) at ($(Ttcs)!0.1!(Btcs)$);
	\coordinate (ReqEnd) at ($(Ttcs)!0.9!(Btcs)$);
	\draw[thick, ->] (ReqStart) -- (ReqEnd) node [above=-.05cm, midway, sloped] {\small(1) Request};
	\coordinate (RepStart) at ($(Btce)!0.1!(Ttce)$);
	\coordinate (RepEnd) at ($(Btce)!0.9!(Ttce)$);
	\draw[thick, ->] (RepStart) -- (RepEnd) node [above=-.05cm, midway, sloped] {\small(3) Report};
\end{tikzpicture}

